A Spectral Algorithm for List-Decodable Covariance Estimation in Relative Frobenius Norm

We study the problem of list-decodable Gaussian covariance estimation. Given a multiset $T$ of $n$ points in $\mathbb R^d$ such that an unknown $\alpha<1/2$ fraction of points in $T$ are i.i.d. samples from an unknown Gaussian $\mathcal{N}(\mu, \Sigma)$, the goal is to output a list of $O(1/\alpha)$ hypotheses at least one of which is close to $\Sigma$ in relative Frobenius norm. Our main result is a $\mathrm{poly}(d,1/\alpha)$ sample and time algorithm for this task that guarantees relative Frobenius norm error of $\mathrm{poly}(1/\alpha)$. Importantly, our algorithm relies purely on spectral techniques. As a corollary, we obtain an efficient spectral algorithm for robust partial clustering of Gaussian mixture models (GMMs) -- a key ingredient in the recent work of [BDJ+22] on robustly learning arbitrary GMMs. Combined with the other components of [BDJ+22], our new method yields the first Sum-of-Squares-free algorithm for robustly learning GMMs. At the technical level, we develop a novel multi-filtering method for list-decodable covariance estimation that may be useful in other settings.

==> GMM_sketch.tex <==

\section{Applications to Learning Gaussian Mixture Models} %
\label{sec:gaussian_mixture_models}

We show the first two bullets as a direct corollary of \Cref{thm:intro} applied to each Gaussian component $D=\cN(\mu_p,\Sigma_p)$ as the inlier distribution.
The proof of the final bullet involves some more involved linear algebraic lemmas.
Here we give only the high-level proof of the final bullet, and defer the proof of these individual lemmas to \Cref{sec:linAlgebra}.

\begin{proof}[Proof Sketch]
\textbf{Outline the first bullet}
\end{proof}

We turn to the final bullet of the theorem.
We will show that any two components $p$ and $p'$ that belong to the same set $T_i$ in the output of the algorithm satisfy that $\|\Sigma^{-1/2}\Sigma_p\Sigma^{-1/2}  - \Sigma^{-1/2}\Sigma_{p'}\Sigma^{-1/2}\|_\fr \lesssim \frac{1}{\alpha^5} \log(1/\alpha)$.
Taking the contrapositive yields the final theorem bullet.

\anote{To be rephrased}
Let $H$ be the second moment matrix of this set, that is, $H = \E_{X \sim T_i}[XX^\top]$.

The lemma states that, if there exists a single matrix $H$ that is an approximate square root to both $\Sigma_1$ and $\Sigma_2$, in the sense that $\|I-H^{\dagger/2}\Sigma_{1}H^{\dagger/2}\|_\fr$ and $\|I-H^{\dagger/2}\Sigma_{1}H^{\dagger/2}\|_\fr$ are both upper bounded, then $\Sigma_1$ and $\Sigma_2$ cannot be too far from each other, in that $\Sigma_1 - \Sigma_2$ must also have bounded Frobenius norm.
In fact, this can be generalized to the normalized version $\Sigma^{-1/2}(\Sigma_1 - \Sigma_2)\Sigma^{-1/2}$ for any positive definite matrix $\Sigma$.

For simplicity of the discussion, let us assume for now that $\Sigma = I$.
To show \Cref{lem:closeness_norm}, a natural first idea is to show that, if $\|I-H^{\dagger/2}\Sigma_1H^{\dagger/2}\|_\fr$ is bounded, say by some quantity $\rho$, then so must be $\|HH^\top - \Sigma_1\|_\fr$ by some quantity related to $O(\rho)$, times the operator norm of $\Sigma_1$ for appropriate scaling.
Unfortunately, that is not true: Even for $\Sigma_1 = I$, we can have $H$ being infinity in the first diagonal element and 1s in the other diagonal elements, and $\|I-H^{\dagger/2}\Sigma_1 H^{\dagger/2}\|_\fr$ would only be 1 yet $HH^\top - \Sigma_1$ is infinite in the first dimension.
The crucial observation, then, is that a slightly weaker statement is true: On an orthonormal basis that depends only on $H$ and not on $\Sigma_1$, $HH^\top$ approximates $\Sigma_1$ in most dimensions, namely $d-O(\rho^2)$ many dimensions.
This statement is formally captured by \Cref{lem:diffFrobNew}.
Thus, in these dimensions, we can bound the difference between $\Sigma_1$ and $\Sigma_2$ (in Frobenius norm).
In the rest of the dimensions where $HH^\top$ does not approximate either $\Sigma_1$ or $\Sigma_2$ well, we can bound these dimensions' contribution to the Frobenius norm of $\Sigma_1 - \Sigma_2$ simply by $\max(\|\Sigma_1\|_\op,\|\Sigma_2\|_\op)$ times the number of such dimensions, which is small.
Combining these bounds yields \Cref{lem:closeness_norm} as desired.
